DRESS: Dynamic RESource-reservation Scheme for Congested Data-intensive Computing Platforms

In the past few years, we have envisioned an increasing number of businesses start driving by big data analytics, such as Amazon recommendations and Google Advertisements. At the back-end side, the businesses are powered by big data processing platforms to quickly extract information and make decisions. Running on top of a computing cluster, those platforms utilize scheduling algorithms to allocate resources. An efficient scheduler is crucial to the system performance due to limited resources, e.g. CPU and Memory, and a large number of user demands. However, besides requests from clients and current status of the system, it has limited knowledge about execution length of the running jobs, and incoming jobs' resource demands, which make assigning resources a challenging task. If most of the resources are occupied by a long-running job, other jobs will have to keep waiting until it releases them. This paper presents a new scheduling strategy, named DRESS that particularly aims to optimize the allocation among jobs with various demands. Specifically, it classifies the jobs into two categories based on their requests, reserves a portion of resources for each of category, and dynamically adjusts the reserved ratio by monitoring the pending requests and estimating release patterns of running jobs. The results demonstrate DRESS significantly reduces the completion time for one category, up to 76.1% in our experiments, and in the meanwhile, maintains a stable overall system performance.

==> problem.tex <==
\section{Problem Formulation}
In this paper, 
we consider a Hadoop YARN cluster as a representative computing platform that consists of a resource manager, 
acted as a master for global scheduling, and name nodes, acted as salves that
hosting a set of containers. In general,
a Hadoop YARN cluster is described by a rich resource vector, such as memory and vcores.
Running on name nodes, containers are basic computing units that utilize blocks of resources to execute the tasks.
Table~\ref{table:locations} lists the notations we use in the rest of this paper. 

We consider a set of $n$ jobs, $\{J_1,J_2,...,J_n\}$ are submitted to a Hadoop YARN cluster. 
Each job can be divided and executed as some tasks, such as Map and Reduce tasks. We assign each task a unique id, such as $t_i$. 
All the tasks form into a set $T$ and then, each job can be represented by a subset of $T$.
Depending on the resources that requested by jobs (or we can assume there is a user-defined expected execution length),
we classify them into two categories $H$ and $L$ to represent large and small jobs. Each category reserve of a percentage of total available resources.
Therefore, if $\alpha$ percent are reserved for small jobs, $1-\alpha$ percent would be available for large jobs.
Assume there are $m$ servers in the cluster, $\{S_1, S_2,...,S_m\}$, each of them has a certain amount of resources in $k$ types
$r_1, r_2,...,r_k$. 
Currently, the Hadoop YARN cluster only consider two types of resources, memory, and CPU. We use $k$ types of resources
in a general setting for potential extensions can involve other types of resources, e.g., network bandwidth and disk I/O. 
In the rest of paper, we use $r_1, r_2$ to denote memory and CPU resources, respectively.

In the cluster, we use a two-dimensional matrix $C$ to monitor each server.
$C[i,j]$ indicates the amount of available resources $r_i$ on server $S_j$, where $i\in [i,k]$ 
and $j\in [1,n]$. The resource manager maintains the matrix and keeps updating through the periodic heartbeat messages from node managers.

In Hadoop YARN, each task can request user-specified resources. All tasks in the same phase (map/reduce) of a job share the same resource demands. 
For a task $t_i \in T$, $RC[i,j]$ represents the demand of the resource $r_j$ requested by $t_i$, where $RC[p,j] = RC[q,j]$ if $t_p$ and $t_q$ are the same type of tasks from the same job. A task $t_i$ can be assigned to a sever $S_j$ as long as $\forall p \in [1,k], RC[i,p] \leq C[i,j]$. Given $C$ and $RC$, our objective is to assign appropriate resources for each category of jobs and design efficient scheduler to minimize the overall execution times of all the jobs (i.e., minimize the makespan). Specifically, let $st_i$ and $\mu_i$ be the starting time and the execution time of a task $t_i$, $t_i \in T$. Let $x_{ij}$ show the association between $t_i$ and $S_j$. $x_{ij}$ is 1 if $t_i$ is assigned to $S_j$. Otherwise, $x_{ij}$ is 0. In this case, our scheduling problem is to derive $st_i$, $x_{ij}$ and $\alpha$ in order to
\vspace{-0.05in}
\begin{eqnarray*}
minimize: max \{st_i + \mu_i\} , \forall i \in T
\end{eqnarray*}
\begin{eqnarray}
&& s.t. \sum_{j \in [1,m]} x_{ij} = 1 , \forall t_i \in T;\\
&& \sum_{t_i \in T} x_{ij}RC[i,p] \leq C[j,p];  \\
&& \sum_{j \in [1,m]} \sum_{t_i \in H(\sigma)} x_{ij}RC[i,p] \leq \alpha * \sum_{j \in [1,m]} C[j,p];\\
&& \sum_{j \in [1,m]} \sum_{t_i \in L(\sigma)} x_{ij}RC[i,p] \leq (1-\alpha) * \sum_{j \in [1,m]} C[j,p];
\end{eqnarray}
\begin{eqnarray*}
x_{ij} \in \{0,1\},  st_i \geq 0, \forall i,j; p \in [1,k], \sigma > 0.	
\end{eqnarray*}

We consider time cost is measured as discrete value which is multiple of the time units. $\sigma$ here represents a particular time point. $H(\sigma)$ and $L(\sigma)$ are defined as the sets of active tasks for large and small jobs at time $\sigma$, i.e., $H(\sigma) = \{ t_i \in H | st_i \leq \sigma \leq st_i + \mu_i\}$ and 
$L(\sigma)  =  \{ t_i \in L | st_i \leq \sigma \leq st_i + \mu_i\}$. Therefore, constrain (1) indicates that a task can be only assigned to one server. Constrain (2) specifies that the resource demands of the activate tasks in one server cannot exceed the resource capacity of that server. And constrain (3) and (4) limit the reserved resources for the jobs in each category. Assume $\mu_i$ is available and each map/reduce task is independent, our scheduling problem is equivalent to general resource constrained scheduling problem which has been proven to be NP-complete~\cite{NP}. There are many heuristics have been proposed to solve this problem and the main challenge is that the execution time of each task is hard to predict. The existing heuristics such as~\cite{aria} and~\cite{polo11} are based on the profiling of tasks execution which in practice, however, cannot be known before they are executed in the system. In this paper, we propose a more practical heuristic that does not require any prior knowledge of the task execution times. 

%In our problem setting, a Yarn cluster
%is running to accept clients' jobs and store them into a queue waiting for execution.
%The cluster has a total resource limited, $R = \{V, M\}$, where $V$ is a number of vcores and $M$ is maximum memory size. 
%Let $J$ represents a set of jobs, $J=\{J_1,J_2,...,J_n\}$. Each job, $J_i \in J$ is
%configured with multiple tasks ($T_i$) 
%To complete a job, $J_i$, it requires to execute a set of tasks, $t_{i1}, t_{i2}, ..., t_{in} \in T_i$
%Each task should request a container from the resource manager. 
%Such a container is dedicated to a particular task until it finishes the execution.
%The containers that allocate to $J_i$ are identical and they can be represented by $C_{i}$, which wrap the resources $<v_i, m_i>$, where
%$v_i$ and $m_i$ are a subset of $V$ and $M$.
\vspace{-0.1in}
%When container finishes executing a task, it releases the resources to Yarn cluster. 
\begin{table}[ht]
\caption{Notation Table}
 \centering
 \small
 \begin{tabular}{c l}
  \hline\hline
  %added by Jiayin
  $J/ S$ & set of jobs/ set of servers in the cluster \\
  \hline
  $n/m$ & number of jobs/work servers in the cluster \\
  \hline
  $T/H/L$ & set of tasks of all jobs/large jobs/small jobs \\
  \hline
  $H(\sigma)/L(\sigma)$ & sets of active tasks for large/small jobs at time $\sigma$\\
  \hline
  $k$ & number of resource types in the work server \\
  \hline
  $C[i,j]$ & the amount of available resources $r_i$ on server $S_j$ \\
  \hline
  $RC[i,j]$ & the amount of resource $r_j$ demanded by task $t_i$ \\
  %added by Jiayin
  %$J / K $ & set of jobs / set of active jobs \\
  \hline
  $RC$ & total resources in the cluster \\
  \hline
  $J_i$ & the $i^{th}$ job in $J$ \\
  \hline
%  $C_i$   &    number of containers dedicated to $J_i$ \\
%  \hline
%  $<v_i, m_i>$    & size of a container for job $J_i$ \\
%  \hline
%  $T_i$    &    number of tasks for $J_i$  \\
%  \hline
%  $T_{ij}$  & the $j^{th}$ task in $T_i$  \\
%  \hline 
%  $F_o$  & observed resource release frequency \\
%  \hline
%  $A_o$   & observed available resources \\
%  \hline
%  $F_e$  & expected resources release frequency\\
%  \hline
%  $A_e$   & observed available resources \\
%  \hline
%  $P$   & number of pending jobs \\
%  \hline
%  $P_R$ &  number of pending resource requests \\
%  \hline
  \hline
\label{table:locations}
\end{tabular}
\end{table}



==> system.tex <==
\section{System Architecture}
\label{system}
In this section, we discuss the framework of \sol.
It contains four major components, 
Client Request Analyst, Running Task Tracker, System Resource Partitioner, and Pending Job Tracker.
In order to reduce the processing overhead, these components of \sol~ are integrated into existing modules in the Resource Manager (RM) of current YARN platform.
Fig~\ref{fig:dress} illustrates the system design. The boxes in purple represent the components in \sol~ and blue boxes are existing modules in RM. 


\begin{figure}[ht]
\centering
\includegraphics[width=0.8\linewidth]{dress}
\caption{Major components in \sol }
\label{fig:dress} 
\end{figure}

{\bf Client Request Analyst}:
The Client Request Analyst (CRA) is implemented in the ClientRMService, which is a module in RM to handle job requests from clients. 
A system administrator configures a specific criterion that is used to classify jobs into different categories.  
The criteria varies depending on settings, such as the amount of requested resources, expected occupation length, and user-specified priorities. 
After analyzing, CRA directs the coming jobs to system scheduler. If the scheduler approves the resource request, it goes to the RMAppManager.

{\bf Pending Job Tracker}:
The Pending Job Tracker(PJT) resides in the System Scheduler that is a manager for all resources in the cluster. 
The jobs from the ClientRMService will be divided into two categories each category has its own resource pool as well as allocation policy.
If the requested resource is not immediately available, the jobs will be managed by PJT. When the resource becomes available, 
PTJ sorts the pending jobs and assigns the resources to them.
Another key function for PJT is to decide the reserve ratio for each category by analyzing both pending and running jobs, which we will discuss in Section~\ref{algorithms}.

{\bf System Resource Partitioner}:
The System Resource Partitioner(SRP) acts as a component of the RMAppManager, which is a system module that manages the list of applications for the RM.
The SRP obtains the reserve ratio from System Scheduler, collects and maintains the resources for each category according to the ratio.
When a job approved by System Scheduler and submitted by the ClientRMService, the RMAppManager will use the resources in a particular partition 
to launch the Application Master(AM) for this job.

{\bf Running Task Tacker}:
The Running Task Tacker(RTT) contains in Application Master Service that gathers the current states from all AMs through enriched heartbeats. 
The RTT creates a table for each job and maintains the progress of their tasks. 
This table is used to estimate the resource release pattern of the system that will help the System Scheduler managing an overall resource 
allocation scheme and making decisions for each job. We will discuss the estimation functions in Section~\ref{solution}.




